Stochastic Volterra Equations for Local Times of Spectrally Positive L\'evy Processes with Gaussian Components

Following our previous work [68], this paper continues to investigate the evolution dynamics of local times of spectrally positive L\'evy processes with Gaussian components in the spatial direction. We prove that conditioned on the finiteness of the first time at which the local time at zero exceeds a given value, local times at positive line are equal in law to the unique solution of a stochastic Volterra equation driven by a Gaussian white noise and two Poisson random measures with convolution kernel given in terms of the scale function. Also, we obtain several equivalent stochastic equations by using the potential theoretic techniques and prove the strong existence and uniqueness by using the generalized Yamada-Watanabe theorems. Armed with the stochastic Volterra representation, we then establish a comparison principle for the local times of spectrally positive L\'evy processes with various drifts or stopped when local times at zero exceed different given values, which proposes a stochastic flow enjoying the branching property. And also, we explore some novel properties of local times in the spatial direction including uniform moment estimates, $(1/2-\varepsilon)$-H\"older continuity and maximal inequality. By using the method of duality, we provide an exponential-affine representation of the Laplace functional in terms of the unique non-negative solution of a path-dependent nonlinear Volterra equation associated with the Laplace exponent of L\'evy process. This gives another perspective on the evolution dynamics of local times in the spatial direction.

==> Comparison.tex <==
  \section{Comparison principle}
 \label{Sec.MainR}
 \setcounter{equation}{0}

==> LaplaceFunctionals.tex <==
 \section{Laplace functionals and weak uniqueness}
 \label{Sec.LaplaceFunctionals}
 \setcounter{equation}{0}
 
 For convenience, we assume that the process $L^\xi_\zeta$, the PRM $\widetilde{N}_\alpha(ds,dy,dz)$ are defined on a filtrated probability basis $(\Omega, \mathscr{G},\mathscr{G}_r,\mathbf{P})$ satisfying the general hypotheses and $N_0(dy,dz)$ is $\mathscr{G}_0$-measurable\footnote{Otherwise, by the definition of weak solutions of (\ref{MainThm.SVE}); see footnote~\ref{Def.WeakSolution}, a realization of $L^\xi_L$, $N_0(dy,dz)$ and $\widetilde{N}_\alpha(ds,dy,dz)$ can be found on some filtrated probability basis such that (\ref{MainThm.SVE}) holds. }.
 For each $\lambda \geq 0$ and $g\in L^\infty(\mathbb{R}_+;\mathbb{R}_+)$, we assume that $(v_\lambda^g,T)$ is a $\mathcal{A}$-local solution of (\ref{MainThm.Volterra}), i.e., $T>0$ and $v_\lambda^g \in \mathcal{A}_{T,J}$ for some $J>0$. 
 For $x,r\geq 0$, conditionally on  $\mathscr{F}_r$ we take expectations on both sides of (\ref{MainThm.SVE}) and get 
 \beqnn
 \mathbf{E}\big[ X_\zeta(x)\,\big|\, \mathscr{F}_0 \big] 
 \ar=\ar \zeta\cdot c\cdot W'(x)  
 +  \int_0^\zeta\int_0^\infty \nabla_yW(x)  \, N_0(dz, dy)
 \eeqnn
 and
 \beqnn
 \mathbf{E}\big[ X_\zeta(x)\,\big|\, \mathscr{F}_r \big] 
 \ar=\ar \mathbf{E}\big[ X_\zeta(x)\,\big|\, \mathscr{F}_0 \big] + \int_0^{r\wedge x} \int_0^{X_\zeta(s)}  W'(x-s) \, B_c(ds,dz) \cr
 \ar\ar + \int_0^{r\wedge x} \int_0^{X_\zeta(s)} \int_0^\infty \nabla_yW(x-s)\, \widetilde{N}_\nu(ds,dz,dy).
 \eeqnn  
 and 
 \beqnn
 \mathbf{E}\big[ X_\zeta(x) \big] 
 \ar=\ar \zeta\cdot \big(1-bW(x)  \big). 
 \eeqnn

 
 \begin{proposition} \label{MartingaleReProp}
  For each $x\geq 0$, the random variable 
  \beqlb
  \mathbf{Y}_x:=  \lambda\cdot  X_\zeta(x)+  \big(g-\boldsymbol{\mathcal{R}}_0\circ V^g_\lambda\big)  *X_\zeta(x) \eeqlb
  is integrable and can be written as
  \beqnn
  \mathbf{Y}_x \ar=\ar Y_x(0)  + \int_0^x \int_0^{X_\zeta(s)}   V^g_\lambda(x-s) \, B_c(ds,dz) \cr
  \ar\ar + \int_0^x\int_0^{X_\zeta(s)} \int_0^\infty \Big( \int_{(x-s-y)^+}^{x-s} V^g_\lambda(r)\,dr\Big) \, \widetilde{N}_\nu(ds,dz,dy),\cr
  Y_x(0)\ar:=\ar   \zeta\cdot c \cdot  V^g_\lambda(x)+ \int_0^\zeta \int_0^\infty \Big( \int_{(x-y)^+}^{x} V^g_\lambda(r)\,dr\Big) N_0(dz,dy).  \label{eqn.900}
  \eeqnn 
 \end{proposition}
 \proof The integrability of $\mathbf{Y}_x$ follows directly from Lemma~?? and the locally uniform boundedness of $g$ and $ \boldsymbol{\mathcal{R}}_0\circ V^g_\lambda $. 
 By ????, we can write $\mathbf{Y}_x$ as the sum of the following three terms   
 \beqnn
 \mathbf{Y}_x^{(1)}\ar:=\ar \lambda \cdot \mathbf{E}\big[ X_\zeta(x)\,\big|\, \mathscr{F}_0 \big] + \int_0^x \big(g-\boldsymbol{\mathcal{R}}_0\circ V^g_\lambda\big) (x-r) \mathbf{E}\big[ X_\zeta(r)\,\big|\, \mathscr{F}_0 \big] \, dr, \cr
  \mathbf{Y}_x^{(2)}\ar:=\ar \int_0^{x} \int_0^{X_\zeta(s)} \lambda \cdot W'(x-s) \, B_c(ds,dz) \cr
  \ar\ar + \int_0^x \big(g-\boldsymbol{\mathcal{R}}_0 \circ V^g_\lambda\big) (x-r) \int_0^{r} \int_0^{X_\zeta(s)} \lambda \cdot W'(r-s) \, B_c(ds,dz) \, dr, \cr 
  \mathbf{Y}_x^{(3)}\ar:=\ar \int_0^{x} \int_0^{X_\zeta(s)} \int_0^\infty  \lambda \cdot \nabla_yW(x-s)\, \widetilde{N}_\nu(ds,dz,dy)\cr
  \ar\ar + \int_0^x \big(g-\boldsymbol{\mathcal{R}}_0\circ V^g_\lambda\big) (x-r) \int_0^{r} \int_0^{X_\zeta(s)} \int_0^\infty  \lambda \cdot \nabla_yW(r-s)\, \widetilde{N}_\nu(ds,dz,dy)\,dr . 
 \eeqnn
 By plugging ?? into $\mathbf{Y}_x^{(1)}$, we first have  
 \beqnn
 \mathbf{Y}_x^{(1)}\ar=\ar \lambda \cdot \mathbf{E}\big[ X_\zeta(x)\,\big|\, \mathscr{F}_0 \big] + \int_0^x \big(g-\boldsymbol{\mathcal{R}}_0\circ V^g_\lambda\big) (x-r) \mathbf{E}\big[ X_\zeta(r)\,\big|\, \mathscr{F}_0 \big] \, dr\cr
 \ar=\ar \lambda \cdot \zeta\cdot c\cdot \Big( W'(x) +   \big(g-\boldsymbol{\mathcal{R}}_0\circ V^g_\lambda\big) * W'(x)  \Big)  +  \int_0^\zeta\int_0^\infty \lambda \cdot \nabla_yW(x)  \, N_0(dz, dy)  \cr
 \ar\ar + \int_0^x \big(g-\boldsymbol{\mathcal{R}}_0\circ V^g_\lambda\big) (x-r) \cdot \int_0^\zeta\int_0^\infty   \nabla_yW(r)  \, N_0(dz, dy) \, dr .
 \eeqnn
 By ???, the first term on the right side of the second equality equals to $\lambda \cdot \zeta\cdot c\cdot V^g_\lambda(x)$. 
 Using the stochastic Fubini theorem along with the locally uniform boundedness of $g$ and $ \boldsymbol{\mathcal{R}}_0\circ V^g_\lambda $ to the last term, it equals to
 \beqnn
 \lefteqn{ \int_0^\zeta\int_0^\infty \int_0^x  \big(g-\boldsymbol{\mathcal{R}}_0\circ V^g_\lambda\big)(x-r) \int_{r-y}^rW'(s)\, ds  \, dr \, N_0(dz, dy) }\ar\ar\cr
  \ar=\ar \int_0^\zeta\int_0^\infty  \int_{x-y}^x   \big(g-\boldsymbol{\mathcal{R}}_0\circ V^g_\lambda\big)* W'(r)  \,dr \, N_0(dz, dy) 
 \eeqnn
 Taking this back into ??, merging it with the second term and then using ???, we have 
 \beqnn
 \mathbf{Y}_x^{(1)}\ar=\ar \lambda \cdot \zeta\cdot c\cdot V^g_\lambda(x) + \int_0^\zeta\int_0^\infty  \int_{x-y}^x V^g_\lambda(r)  \,dr \, N_0(dz, dy). 
 \eeqnn
 Similarly, applying the stochastic Fubini theorem to the second terms in $ \mathbf{Y}_x^{(2)}$ and $ \mathbf{Y}_x^{(3)}$ we also have 
 \beqnn
 \lefteqn{\int_0^x \big(g-\boldsymbol{\mathcal{R}}_0\circ V^g_\lambda\big) (x-r) \int_0^{r} \int_0^{X_\zeta(s)} \lambda \cdot W'(r-s) \, B_c(ds,dz) \, dr}\ar\ar\cr
 \ar=\ar \int_0^x  \int_0^{X_\zeta(s)} \lambda \cdot  \big(g-\boldsymbol{\mathcal{R}}_0\circ V^g_\lambda\big) * W'(x-s) \, B_c(ds,dz)  
 \eeqnn
 and 
 \beqnn
 \lefteqn{\int_0^x \big(g- \boldsymbol{\mathcal{R}}_0\circ V^g_\lambda\big) (x-r) \int_0^{r} \int_0^{X_\zeta(s)} \int_0^\infty  \lambda \cdot \nabla_yW(r-s)\, \widetilde{N}_\nu(ds,dz,dy)\,dr }\ar\ar\cr
 \ar=\ar \int_0^x  \int_0^{X_\zeta(s)} \int_0^\infty  \lambda \cdot \int_{x-s-y}^{x-s}\big(g- \boldsymbol{\mathcal{R}}_0\circ V^g_\lambda\big)*W'(r)dr\, \widetilde{N}_\nu(ds,dz,dy).
 \eeqnn
 Plugging them back into ??? and ?? and then merging with 
 \beqnn
  \mathbf{Y}_x^{(2)}\ar:=\ar \int_0^{x} \int_0^{X_\zeta(s)}  V^g_\lambda(x) \, B_c(ds,dz), \cr 
 \mathbf{Y}_x^{(3)}\ar:=\ar \int_0^{x} \int_0^{X_\zeta(s)} \int_0^\infty  \int_{x-s-y}^{x-s} V^g_\lambda(r)\,dr\, \widetilde{N}_\nu(ds,dz,dy).
 \eeqnn
 The desired representation follows by putting ???-??? together.
 \qed 
 
% \begin{proposition}
% 	For each $x\geq 0$, the following hold. 
% 	\begin{enumerate}
% 		\item[(1)] The random variable $\mathbf{Y}_x:=  \lambda\cdot  X_\zeta(x)+ g *  X_\zeta(x) - (\boldsymbol{\varPhi}_0\circ V^g_\lambda)  *X_\zeta(x) $ can be written as
% 		\beqnn
% 		\mathbf{Y}_x \ar=\ar Y_x(0)  + \int_0^x \int_0^{X_\zeta(s)}   V^g_\lambda(x-s) \, B_c(ds,dz) \cr
% 		\ar\ar + \int_0^x\int_0^{X_\zeta(s)} \int_0^\infty \Big( \int_{(x-s-y)^+}^{x-s} V^g_\lambda(r)\,dr\Big) \, \widetilde{N}_\nu(ds,dz,dy),\cr
% 		Y_x(0)\ar:=\ar   \zeta\cdot c \cdot  V^g_\lambda(x)+ \int_0^\zeta \int_0^\infty \Big( \int_{(x-y)^+}^{x} V^g_\lambda(r)\,dr\Big) N_0(dz,dy).  \label{eqn.900}
% 		\eeqnn
% 		
% 		\item[(2)] 
% 	\end{enumerate}
% 	
% \end{proposition}
% \proof The first claim follows directly from Lemma~??? and the locally uniform boundedness of $g$ and $ \boldsymbol{\varPhi}_0\circ V^g_\lambda $, i.e., 
% \beqnn
% \mathbf{E}\Big[\big|Y_x(x)\big|\Big]:=  \lambda\cdot  \mathbf{E}\Big[\big|X_\zeta(x)\big|\Big]+ \Big(\|g\|_{L^\infty_x} + \big\|\boldsymbol{\varPhi}_0\circ V^g_\lambda \big\|_{L^\infty_x}\Big)\cdot \int_0^x \mathbf{E}\Big[\big|X_\zeta(s)\big|\Big]ds  <\infty.
% \eeqnn
% For the second claim, by (???) we have 
%  \beqnn
% Y_x(0)\ar=\ar\mathbf{E}\big[ Y_x(x) \,\big|\,  \mathscr{F}_0\big] 
% = \lambda \cdot \mathbf{E}\big[L^\xi_\zeta(x) \,\big|\,  \mathscr{F}_0\big] 
% + \int_0^x \Big( g- \boldsymbol{\varPhi}_0\circ V^g_\lambda \Big)(x-r) \mathbf{E}\big[L^\xi_\zeta(r)\,\big|\,  \mathscr{F}_0\big]dr\cr
% \ar=\ar \lambda \cdot \zeta\cdot c\cdot W'(x)   +  \int_0^x \Big( g- \boldsymbol{\varPhi}_0\circ V^g_\lambda \Big)(x-r) \cdot  \lambda \cdot \zeta\cdot c\cdot W'(x)dr
%  \cr
% \ar\ar + \int_0^\zeta\int_0^\infty  \lambda \cdot \nabla_yW(x)  \, N_0(dz, dy)  +  \int_0^x \Big( g- \boldsymbol{\varPhi}_0\circ V^g_\lambda \Big)(x-r)   \int_0^\zeta\int_0^\infty \nabla_y W(r) \, N_0(dz, dy) dr \cr
% \ar=\ar  \zeta\cdot c \cdot \bigg(\lambda \cdot W'(x)  +  \int_0^x \Big( g- \boldsymbol{\varPhi}_0\circ V^g_\lambda \Big)(x-r) \cdot   W'(r) dr\bigg) \cr
% \ar\ar + \lambda \cdot \int_0^\zeta\int_0^\infty \nabla_y W(x) \, N_0(dz, dy) 
% +  \int_0^x \Big( g- \boldsymbol{\varPhi}_0\circ V^g_\lambda \Big)(x-r)   \int_0^\zeta\int_0^\infty \nabla_y W(r) \,N_0(dz, dy) dr \cr
% \ar=\ar \zeta\cdot c \cdot  V^g_\lambda(x)  + \int_0^\zeta\int_0^\infty \Big( \int_{(x-y)^+}^x V^g_\lambda (r)dr \Big) \, N_0(dz, dy)
% \eeqnn
% 
% We first have 
% \beqnn
% X_\zeta(x)\ar=\ar \mathbf{E}\big[ X_\zeta(x)\,\big|\, \mathscr{F}_0 \big] 
% + \int_0^{x} \int_0^{X_\zeta(s)}  W'(x-s) \, B_c(ds,dz) \cr
% \ar\ar + \int_0^{x} \int_0^{X_\zeta(s)} \int_0^\infty  \nabla_y W(x-s) \, \widetilde{N}_\nu(ds,dz,dy)
% \eeqnn
% and then
% \beqnn
% Y_x(x)
% \ar=\ar 
% \lambda \cdot \mathbf{E}\big[ X_\zeta(x)\,\big|\, \mathscr{F}_0 \big] 
% + \int_0^{x} \int_0^{X_\zeta(s)} \lambda \cdot W'(x-s) \, B_c(ds,dz) \cr
% \ar\ar + \int_0^{x} \int_0^{X_\zeta(s)} \int_0^\infty  \lambda \cdot \nabla_y W(x-s) \, \widetilde{N}_\nu(ds,dz,dy)\cr
% \ar\ar +  \int_0^x \big( g - \boldsymbol{\varPhi}_0\circ V^g_\lambda \big)(x-r)  \mathbf{E}\big[ X_\zeta(r)\,\big|\, \mathscr{F}_0 \big] dr \cr
% \ar\ar + \int_0^x \big( g - \boldsymbol{\varPhi}_0\circ V^g_\lambda \big)(x-r)\int_0^{r} \int_0^{X_\zeta(s)}  W'(r-s) \, B_c(ds,dz)\, dr\cr
% \ar\ar + \int_0^x \big( g - \boldsymbol{\varPhi}_0\circ V^g_\lambda \big)(x-r) \int_0^{r} \int_0^{X_\zeta(s)} \int_0^\infty  \nabla_y W(r-s) \, \widetilde{N}_\nu(ds,dz,dy)\,dr \cr
% \ar=\ar \lambda \cdot \mathbf{E}\big[ X_\zeta(x)\,\big|\, \mathscr{F}_0 \big] 
% +  \int_0^x \big( g - \boldsymbol{\varPhi}_0\circ V^g_\lambda \big)(x-r)  \mathbf{E}\big[ X_\zeta(r)\,\big|\, \mathscr{F}_0 \big] dr \cr 
% \ar\ar + \int_0^{x} \int_0^{X_\zeta(s)} \Big[ \lambda \cdot W'(x-s)  + \big( g - \boldsymbol{\varPhi}_0\circ V^g_\lambda \big)*W'(x-s)\Big] \, B_c(ds,dz)\,  \cr
% \ar\ar + \int_0^x   \int_0^{X_\zeta(s)} \int_0^\infty \Big[  \lambda \cdot \nabla_y W(x-s) + \big( g - \boldsymbol{\varPhi}_0\circ V^g_\lambda \big) * \big(\nabla_y W\big)(x-s) \Big]\, \widetilde{N}_\nu(ds,dz,dy)\,dr 
% \eeqnn
% 
% Let 
% \beqnn
% Y_x(x):= \lambda \cdot L^\xi_\zeta(x) +  \Big( g- c \cdot \big|V^g_\lambda\big|^2 -\mathcal{V}\circ V^g_\lambda \Big)* L^\xi_\zeta(x)
% \eeqnn
% and 
% \beqnn
% \mathbf{E}\big[ Y_x(x) \big]\ar=\ar \lambda \cdot \mathbf{E}\big[L^\xi_\zeta(x)\big] +  \Big( g- c \cdot \big|V^g_\lambda\big|^2 -\mathcal{V}\circ V^g_\lambda \Big)* \mathbf{E}\big[L^\xi_\zeta(\cdot)\big](x)\cr
% \ar=\ar \zeta \bigg( \lambda \cdot \big( 1-b\cdot W(x) \big) + \Big( g- c \cdot \big|V^g_\lambda\big|^2 -\mathcal{V}\circ V^g_\lambda \Big)* \big( 1-b\cdot W\big) (x)  \bigg)
% \eeqnn
% 
% For any $t\in [0,x]$,
% \beqnn
% Y_x(t):=\mathbf{E}\big[ Y_x(x) \,\big|\,  \mathscr{F}_t\big] 
% \ar=\ar  \lambda \cdot \mathbf{E}\big[L^\xi_\zeta(x) \,\big|\,  \mathscr{F}_t\big] +  \Big( g- c \cdot \big|V^g_\lambda\big|^2 -\mathcal{V}\circ V^g_\lambda \Big)* \mathbf{E}\big[L^\xi_\zeta(\cdot)\,\big|\,  \mathscr{F}_t\big](x) \cr
% \ar=\ar \lambda \cdot \mathbf{E}\big[L^\xi_\zeta(x) \,\big|\,  \mathscr{F}_t\big] + \int_0^x \Big( g- c \cdot \big|V^g_\lambda\big|^2 -\mathcal{V}\circ V^g_\lambda \Big)(x-r) \mathbf{E}\big[L^\xi_\zeta(r)\,\big|\,  \mathscr{F}_t\big]dr
% \eeqnn
% and 
%
% and 
% \beqnn
% Y_x(t) 
% \ar=\ar \lambda \cdot \mathbf{E}\big[L^\xi_\zeta(x) \,\big|\,  \mathscr{F}_t\big] + \int_0^x \Big( g- c \cdot \big|V^g_\lambda\big|^2 -\mathcal{V}\circ V^g_\lambda \Big)(x-r) \mathbf{E}\big[L^\xi_\zeta(r)\,\big|\,  \mathscr{F}_t\big]dr\cr
% \ar=\ar Y_x(0) 
% + \lambda \cdot \int_0^{t } \int_0^{L^\xi_\zeta(s)}  W'(x-s) \, B(ds,dz)  
% + \lambda \cdot\int_0^{t} \int_0^{L^\xi_\zeta(s)} \int_0^\infty  \nabla_y W(x-s)\, \widetilde{N}_1(ds,dz,dy) \cr
% \ar\ar + \int_0^x \Big( g- c \cdot \big|V^g_\lambda\big|^2 -\mathcal{V}\circ V^g_\lambda \Big)(x-r)  \int_0^{t\wedge r} \int_0^{L^\xi_\zeta(s)}   W'(r-s) \, B(ds,dz)  dr\cr
% \ar\ar + \int_0^x \Big( g- \frac{\sigma^2}{2} \cdot \big|V^g_\lambda\big|^2 -\mathcal{V}\circ V^g_\lambda \Big)(x-r) \int_0^{t\wedge r} \int_0^{L^\xi_\zeta(s)} \int_0^\infty  \nabla_y W(r-s)\, \widetilde{N}_1(ds,dz,dy) dr\cr
% \ar=\ar Y_x(0) 
% + \int_0^{t } \int_0^{L^\xi_\zeta(s)}   \lambda \cdot  W'(x-s) \, B(ds,dz) \cr
% \ar\ar 
% + \int_0^{t } \int_0^{L^\xi_\zeta(s)}  \Big( g- c \cdot \big|V^g_\lambda\big|^2 -\mathcal{V}\circ V^g_\lambda \Big) *W'(x-s) \, B(ds,dz)  \cr
% \ar\ar + \int_0^{t} \int_0^{L^\xi_\zeta(s)} \int_0^\infty  \lambda \cdot\nabla_y W(x-s)\, \widetilde{N}_1(ds,dz,dy)\cr
% \ar\ar + \int_0^{t} \int_0^{L^\xi_\zeta(s)} \int_0^\infty \Big( g- c \cdot \big|V^g_\lambda\big|^2 -\mathcal{V}\circ V^g_\lambda \Big) *\nabla_y W(x-s)\, \widetilde{N}_1(ds,dz,dy) \cr
% \ar=\ar Y_x(0)  
% +    \int_0^{t } \int_0^{L^\xi_\zeta(s)}  \bigg(\lambda \cdot  W'(x-s) + \Big( g- c \cdot \big|V^g_\lambda\big|^2 -\mathcal{V}\circ V^g_\lambda \Big) *W'(x-s)\bigg) \, B(ds,dz)  \cr
% \ar\ar + \int_0^{t} \int_0^{L^\xi_\zeta(s)} \int_0^\infty \bigg( \lambda \cdot\nabla_y W(x-s)+ \Big( g- c \cdot \big|V^g_\lambda\big|^2 -\mathcal{V}\circ V^g_\lambda \Big) *\nabla_y W(x-s) \bigg)\, \widetilde{N}_1(ds,dz,dy) \cr
% \ar=\ar Y_x(0)  
% +  \sigma \cdot \int_0^{t } \int_0^{L^\xi_\zeta(s)}  V^g_\lambda(x-s) \, B(ds,dz)  + \int_0^{t} \int_0^{L^\xi_\zeta(s)} \int_0^\infty \int_{(x-s-y)^+}^{x-s} V^g_\lambda(r)dr \, \widetilde{N}_1(ds,dz,dy)  
% \eeqnn
% 
% 
% \qed
% 
 Associated to the random variable $\mathbf{Y}_x$ we define a  Doob martingale $Y_x:=\{Y_x(t) : t \in[0,x] \}$ by
 \beqlb
 Y_x(t):= \mathbf{E}\big[\mathbf{Y}_x \big|\mathscr{F}_t\big] .
 \eeqlb
 Taking expectations on both sides of ??? conditionally on $\mathscr{F}_t$,  the martingale $Y_x$ admits the following representation 
 \beqlb  \label{eqn.9000}
 Y_x(t) \ar=\ar Y_x(0) + \int_0^{t} \int_0^{X_\zeta(s)}   V^g_\lambda(x-s) \, B_c(ds,dz)\cr
 \ar\ar  + \int_0^{t} \int_0^{X_\zeta(s)} \int_0^\infty \Big( \int_{(x-s-y)^+}^{x-s} V^g_\lambda(r)\,dr\Big) \, \widetilde{N}_\nu(ds,dz,dy) . 
 \eeqlb
 
 \begin{lemma}
 	The $(\mathscr{F}_t)$-continuous semimartingale $Z_x$ admits the following decomposition
 	\beqlb\label{eqn.9001}
 	Z_x(t) \ar=\ar	Y_x(t) + \int_0^t \boldsymbol{\mathcal{R}}_0\circ V^g_\lambda(x-s) X_\zeta(s)ds,
 	\quad t\in[0,x] . 
 	\eeqlb 
 \end{lemma} 
 \proof  
 %we first have
 %\beqnn
 %\mathbf{E}\Big[  \big(\boldsymbol{\varPhi}_0\circ V^g_\lambda \big)* X_\zeta(x)\,\Big|\, \mathscr{F}_t \Big]
 %\ar=\ar \int_0^t \boldsymbol{\varPhi}_0\circ V^g_\lambda(x-s) X_\zeta(s)\, ds \cr
 %\ar\ar + \int_t^x \boldsymbol{\varPhi}_0\circ V^g_\lambda(x-s) \mathbf{E}\Big[ X_\zeta(s)\,\Big|\, \mathscr{F}_t \Big]\, ds
 %\eeqnn
 Plugging ?? into ???, we have 
 \beqnn
 Y_x(t)
 %\ar=\ar  \mathbf{E}\Big[   \lambda\cdot  X_\zeta(x)+ g *  X_\zeta(x) - (\boldsymbol{\varPhi}_0\circ V^g_\lambda)  *X_\zeta(x) \,\Big|\, \mathscr{F}_t \Big]\cr
 %\ar=\ar \mathbf{E}\Big[   \lambda\cdot  X_\zeta(x)+ g *  X_\zeta(x)\,\Big|\, \mathscr{F}_t \Big] -\mathbf{E}\Big[  (\boldsymbol{\varPhi}_0\circ V^g_\lambda)  *X_\zeta(x) \,\Big|\, \mathscr{F}_t \Big] \cr
 \ar=\ar  \mathbf{E}\big[   \lambda\cdot  X_\zeta(x)+ g *  X_\zeta(x)\,\big|\, \mathscr{F}_t \big]   -\int_0^t \boldsymbol{\mathcal{R}}_0\circ V^g_\lambda(x-s) X_\zeta(s)\, ds \cr
 \ar\ar - \int_t^x \boldsymbol{\mathcal{R}}_0\circ V^g_\lambda(x-s) \mathbf{E}\big[ X_\zeta(s)\,\big|\, \mathscr{F}_t \big]\, ds. 
 \eeqnn
 Moving the second term on the right-hand side to the left-hand side and then comparing it to the definition of $Z_x$, we can get the equality ??? immediately.  
 \qed  
 
 Note  that $Z_x(0)=Y_x(0)$. 
 Applying It\^o's formula (see Theorem 5.1 in \cite[p.66]{IkedaWatanabe1989}) along with \eqref{eqn.9000}-\eqref{eqn.9001} to $e^{-Z_x(t)}$ and then using (????), we have  
 \beqnn 
 e^{-Z_x(t)} 
  %\ar=\ar e^{-Y_x(0)}-\int_0^t   e^{-Z_x(s)}X_\zeta(s)\cdot \boldsymbol{\varPhi}_0\circ V^g_\lambda(x-s)  \, ds \cr
  %\ar\ar - \int_0^{t } \int_0^{L^\xi_\zeta(s)} e^{-Z_x(s)}  V^g_\lambda(x-s) \, B_c(ds,dz) +\int_0^{t }  e^{-Z_x(s)}   X_\zeta(s)\cdot c \big| V^g_\lambda(x-s) \big|^2 \, ds\cr
  %\ar\ar + \int_0^{t} \int_0^{X_\zeta(s)} \int_0^\infty e^{-Z_x(s-)} \Big( \exp\Big\{-\int_{(x-s-y)^+}^{x-s} V^g_\lambda(r)dr\Big\} -1 \Big) \, \widetilde{N}_\nu(ds,dz,dy) \cr
  %\ar\ar + \int_0^{t}  \int_0^\infty  e^{-Z_x(s)} X_\zeta(s) \Big( \exp\Big\{-\int_{(x-s-y)^+}^{x-s} V^g_\lambda(r)dr\Big\} -1 +\int_{(x-s-y)^+}^{x-s} V^g_\lambda(r)dr\Big) \, ds\nu(dy)\cr  
  \ar=\ar e^{-Y_x(0)} + \int_0^{t }   e^{-Z_x(s)} dU_x(s), 
  \quad t\in[0,x], 
 \eeqnn
 where  $U_x:=\big\{U_x(t):t\in[0,x] \big\}$ is a $(\mathscr{F}_t)$-local martingale defined by 
 \beqnn
 U_x(t)\ar:=\ar -  \int_0^{t } \int_0^{ X_\zeta(s)}   V^g_\lambda(x-s) \, B_c(ds,dz) \cr
 \ar\ar  + \int_0^{t} \int_0^{X_\zeta(s)} \int_0^\infty  \Big( \exp\Big\{-\int_{(x-s-y)^+}^{x-s} V^g_\lambda(r)dr\Big\} -1 \Big) \, \widetilde{N}_\nu(ds,dz,dy).
 \eeqnn
 Multiplying both sides of the preceding equalities by a $e^{Y_x(0)}$ yields that the process $\{e^{Y_x(0)-Z_x(t)}:t\in[0,x]\}$ equals to the Dol\'ean-Dade exponential  $\mathcal{E}_{U_x}$ associated to the local martingale $U_x$.  
 
 
 \begin{lemma}
 The Dol\'eans-Dade exponential $\mathcal{E}_{U_x}$ is a true $(\mathscr{F}_t)$-martingale.  
 \end{lemma}
 \proof  
 By It\^o's formula, the stochastic exponential $\mathcal{E}_{U_x}$ admit the following representation
 \beqnn
 \mathcal{E}_{U_x}(t)
 \ar=\ar\exp\Big\{ - \int_0^t \boldsymbol{\mathcal{R}}_0\circ V^g_\lambda (x-s) X_\zeta(s) ds -\int_0^{t } \int_0^{ X_\zeta(s)}   V^g_\lambda(x-s) \, B_c(ds,dz) \cr
 \ar\ar\ \  \quad\quad - \int_0^t \int_0^{X_\zeta(s)}\int_0^\infty  \Big(\int_{(x-s-y)^+}^{x-s} V^g_\lambda(r)dr \Big)  \widetilde{N}_\nu (ds,dz,dy) \Big\}.
 \eeqnn
 Notice that $ \mathcal{E}_{U_x}$ is a non-negative local martingale and hence a supermartingale.
 By Fatou's lemma, we have $\mathbf{E}[\mathcal{E}_{U_x}(t)] \leq 1$ and hence it suffices to identify that $\mathbf{E}[\mathcal{E}_{U_x}(t)]=1$ for any $t\geq 0$.
 For each $t_0\geq 0$ and $n\geq 1$, let 
 \beqnn
 \tau_n:=\inf\big\{ t\geq 0: X_\zeta (t)\geq n \big\} \wedge t_0
 \quad\mbox{and}\quad 
 \mathcal{E}_{U_x}^n(t):=  \mathcal{E}_{U_x}(\tau_n \wedge t),\quad t\geq 0. 
 \eeqnn 
 % By Proposition~\ref{UpBoundVf01}, there exists a constant
 By the inequality $|1+(z-1)e^{z} | \leq z^2e^{z} $ for any $z\in\mathbb{R}$ and Proposition~\ref{UpBoundVf01}, there exists a constant $C>0$ such that for any $t\geq 0$,
 \beqnn
 \ar\ar \int_0^x \mathbf{1}_{\{s\leq \tau_n\}} X_\zeta (s) ds \int_0^\infty \Big| 1-\Big( 1+\int_{(x-s-y)^+}^{x-s}V_\lambda^g(r) dr \Big)     \exp\Big\{- \int_{(x-s-y)^+}^{x-s}V_\lambda^g(r) dr\Big\}  \Big| \nu(dy) \cr
 \ar\leq\ar n \sup_{s\in[0,x]} \int_0^\infty \Big(  \int_{(x-s-y)^+}^{x-s}V_\lambda^g(r) dr\Big)^2 \exp\Big\{- \int_{(x-s-y)^+}^{x-s}V_\lambda^g(r) dr\Big\} \nu (dy) \cr
 \ar\leq\ar C\cdot  \int_0^x s^{\alpha-1}ds  \leq C x^\alpha.
 \eeqnn
 By Theorem~IV.3 in \cite{LepingleMemin1978} with 
 $$y(s,z)= \mathbf{1}_{\{s\leq \tau_n\}}\cdot \bigg(\exp\Big\{- \int_{(x-s-y)^+}^{x-s}v_\lambda^g(r) dr \Big\}-1\bigg),$$
 the process $\mathcal{E}_{U_x}^n$ is a martingale for each $n\geq 1$. Thus
 \beqnn
 1= \mathbf{E}\big[\mathcal{E}_{U_x}^n(t_0)\big]
 \ar=\ar \mathbf{E}\big[\mathcal{E}_{U_x}^n(t_0); \tau_n = t_0\big] + \mathbf{E}\big[\mathcal{E}_{U_x}^n(t_0);\tau_n<t_0\big] \cr
 \ar\ar\cr
 \ar=\ar \mathbf{E}\big[\mathcal{E}_{U_x}(t_0);\tau_n= t_0\big] + \mathbf{E}\big[\mathcal{E}_{U_x}^n(t_0);\tau_n<t_0\big] .
 \eeqnn
 By the monotone convergence theorem and the fact that $\tau_n\overset{\rm a.s.}\to t_0$  as $n\to\infty$, we have 
 $$ \mathbf{E}\big[\mathcal{E}_{U_x}(t_0); \tau_n=t_0\big]\to  \mathbf{E}\big[\mathcal{E}_{U_x}(t_0)\big] .$$
 Thus it suffices to prove that $ \mathbf{E}\big[\mathcal{E}_{U_x}^n(t_0);\tau_n<t_0\big] \to 0$ as $n\to\infty$.
 Associate with the martingale $\mathcal{E}_{U_x}^n$, we define a probability law  $\mathbf{Q}_x^n$ on $(\Omega,\mathscr{G},\mathscr{G}_r)$ by 
 \beqnn
 \frac{d  \mathbf{Q}_x^n}{d \mathbf{P}}= \mathcal{E}_{U_x}^n(\tau_n). 
 \eeqnn
 %such that it absolutely continuous with respect to $\mathbf{P}$ with Radon-Nikodym derivative $\mathcal{E}_{U_x}^n(\tau_n)$.
 %For simplicity, we also denote its expectation by $\mathbf{Q}_n^x$.
 Since $\mathcal{E}_{U_x}^n(0)\overset{a.s.}=1$, the PRM $N_0(dy,dz)$ is $\mathscr{G}_0$-measurable and has the same distribution under $\mathbf{P}$ and $\mathbf{Q}_x^n$.
 By Girsanov's theorem for random measure; see Theorem~3.17 in \cite[p.170]{JacodShiryaev2003}, the PRM $N_\alpha(ds,dy,dz)$ is a random point measure under $\mathbf{Q}_x^n$ with intensity
 \beqnn
 \mathbf{1}_{\{ s\leq \tau_n \}}\cdot \exp\Big\{- \int_{(x-s-y)^+}^{x-s}v_\lambda^g(r) dr\Big\}  ds \cdot \nu_\alpha(dy) \cdot dz,
 \eeqnn
 and the SVE (\ref{MainThm.SVE}) is equal in distribution to the following SVE under  $\mathbf{Q}_x^n$,
 \beqnn
 X_{\zeta}(t)\ar=\ar   X_{\zeta,0}(t) + B^n(t)+ M^n(t),\quad t\geq 0,  %\int_0^\infty  \int_0^\zeta \nabla_y W(t)   N_0( dy,dz)
 % + \int_0^t \int_0^\infty \int_0^{L^\xi_{\zeta,n}(s)}  \nabla_y W(t-s)   \widetilde{N}_\alpha(ds,dy,dz),
 \eeqnn
 where $X_{\zeta,0}$ is defined as in (\ref{MartingaleX}), $ M^n$ is defined as in (\ref{MartingaleM}) with $X_{\zeta} $ replaced by $L^{\xi}_{\zeta} $ and
 \beqnn
 B^n(t)\ar:=\ar \int_0^t   \mathbf{1}_{\{ s\leq \tau_n \}} X_{\zeta}(s)ds  \int_0^\infty  \nabla_y W(t-s) \times \cr
 \ar\ar \times \Big(  \exp\Big\{- \int_{(x-s-y)^+}^{x-s}V_\lambda^g(r) dr\Big\} -1 \Big) \nu (dy).
 \eeqnn
 Proposition~\ref{UpBoundVf01} implies that 
 \beqnn
 \exp \Big\{- \int_{(x-s-y)^+}^{x-s}V_\lambda^g(r) dr \Big\} 
 \eeqnn
 is uniformly bounded in $s,y\geq 0$.
 Similarly as in the proofs of Lemma~\ref{Lemma.501}-\ref{MomentIncreM}, there exists a constant $C>0$ such  that for any $n\geq 1$, $t>0$, $t_1,t_2\in[0,t]$ and $p> 1$,
 \beqlb\label{eqn.418}
 \mathbf{E}^{\mathbf{Q}_x^n} \Big[\big|X_{\zeta,0}(t)\big|^p + \big|X_{\zeta}(t)\big|^p\Big]< C\cdot (1+t)^{p\alpha} 
 \eeqlb
 and
 \beqnn
 \mathbf{E}^{\mathbf{Q}_x^n} \Big[\big|X_{\zeta,0}(t_1)-X_{\zeta,0}(t_2)\big|^p + \big| M^n (t_1)- M^n (t_2)\big|^p\Big]\leq C \cdot (1+t)^{p\alpha}\cdot |t_1-t_2|^{p\alpha}.
 \eeqnn
 Here $\mathbf{E}^{\mathbf{Q}_x^n}$ is the expectation under $ \mathbf{Q}_x^n$.
 Together with these estimates, an argument similar to that in the proof of  Theorem~\ref{Thm.Regularity} implies that for any $\kappa\in(0,\alpha/2)$, both $ X_{\zeta,0} $ and $ M^n  $ are locally $\kappa$-H\"older continuous under $\mathbf{Q}_n^x$ and the H\"older coefficient has finite moments of all orders.
 Like the argument before Corollary~\ref{Cor.Maxi}, we have
 \beqlb\label{eqn.612}
 \sup_{n\geq 1}\mathbf{E}^{\mathbf{Q}_x^n}\Big[\sup_{s\in[0,t]}| X_{\zeta,0}(s)|^p\Big]+ \sup_{n\geq 1}\mathbf{E}^{\mathbf{Q}_x^n}\Big[\sup_{s\in[0,t]}| M^n(s)|^p \Big]<\infty,
 \eeqlb
 for any $t,p\geq 0$.  
 Noting that $ \int_{(x-s-y)^+}^{x-s}v_\lambda^g(r) dr=0$ when $s\geq x$, we have for any $t\geq 0$,
 \beqnn
 B^n(t) 
 \ar =\ar \int_0^{t\wedge x}  \mathbf{1}_{\{ s\leq \tau_n \}} L^\xi_{\zeta}(s)ds  \int_0^\infty  \nabla_y W(t-s) \times \cr
 \ar\ar\times  \Big(  \exp\Big\{- \int_{(x-s-y)^+}^{x-s}v_\lambda^g(r) dr\Big\} -1 \Big) \nu_\alpha(dy).
 \eeqnn
 By H\"older's inequality and Proposition~\ref{UpBoundVf01}, the preceding inner integral can bounded by $C\cdot((x-s)^+ \cdot (t-s)^+)^{(\alpha-1)/2}$ uniformly in $t,s,y>0$.
 By (\ref{eqn.418}) and H\"older's inequality, we have for $p>1$,
 \beqnn
 \lefteqn{\mathbf{E}^{\mathbf{Q}_x^n}\Big[ \sup_{t\geq 0} \big| B^n(t)\big|^p \Big]}\ar\ar\cr
 \ar\leq\ar  C \int_0^{x\wedge t \wedge t_0} \mathbf{E}^{\mathbf{Q}_x^n}\Big[\big|L^\xi_{\zeta}(s)\big|^p\Big]  (x-s)^{\alpha-1}ds  \Big(\int_0^x   (x-r)^{\alpha-1} dr\Big)^{p-1} \leq C\cdot x^{p\alpha},
 \eeqnn
 for some constant $C>0$ independent of $n\geq 1$. This, together with (\ref{eqn.612}), yields that  
 $$\mathbf{E}^{\mathbf{Q}_x^n}\Big[\sup_{s\in[0,t_0]}\big|L^{\xi}_{\zeta}(s)\big|^p \Big]\leq C ,$$ 
 uniformly in $n\geq 1$. 
 By the definition of $\tau_n$ and Chebyshev's inequality,
 \beqnn
 \mathbf{E}\big[\mathcal{E}_{U_x}^n(\tau_n); \tau_n<t_0 \big]  =\mathbf{Q}_x^n \big(\tau_n<t_0 \big) 
 \ar=\ar \mathbf{Q}_x^n\Big(\sup_{s\in[0,t_0]}X_{\zeta} (s)\geq n\Big)\cr \ar\leq\ar \frac{1}{n}\mathbf{E}^{\mathbf{Q}_x^n}\Big[\sup_{s\in[0,t_0]}X_{\zeta} (s)\Big],
 \eeqnn
 which vanishes as $n\to\infty$. Hence $\mathbf{E}[\mathcal{E}_{U_x}(t_0)]=1$ and $\mathcal{E}_{U_x}$ is a $(\mathscr{G}_r)$-martingale under $\mathbf{P}$.
 By Proposition~\ref{UpBoundVf01},
 \beqnn
 \int_0^\infty \Big| 1- \exp\Big\{  - \int_{(x-y)^+}^{x}V_\lambda^g(r) dr \Big\} \Big|\bar\nu (y)dy
 \ar\leq\ar  C \int_0^\infty \Big| \int_{(x-y)^+}^{x}V_\lambda^g(r) dr \Big| \bar\nu (y)dy .
 % \ar\leq\ar C \|v_\lambda^g\|_{L^1_x}  \int_{x/2}^\infty \bar\nu_\alpha(y)dy + C  \int_0^{x/2} \int_{x-y }^{x} \big| v_\lambda^g(r)\big| dr \bar\nu_\alpha(y)dy\cr
 % \ar\leq\ar  C \|v_\lambda^g\|_{L^1_x} \cdot x^{-\alpha}  + C x^{\alpha-1}  \int_0^{x/2} y\bar\nu_\alpha(y)dy <\infty.
 \eeqnn
 Similarly as in the proof for Proposition~\ref{UpBoundVf01}, we can prove that the last quantity is finite.
 From this and the exponential formula for PRMs; see \cite[p.8]{Bertoin1996},
 \beqnn
 \mathbf{E}\big[ \exp\{ - Y_x(0) \} \big] =  \exp \Big\{- \zeta \int_0^\infty \Big(1-\exp\Big\{- \int_{(x-y)^+}^x   V_\lambda^g(s) ds\Big\}\Big)\bar\nu (y)dy \Big\}<\infty.
 \eeqnn
 Notice that $e^{ -Z_x }= e^{ -Y_x(0)}\mathcal{E}_{U_x} $ on $[0,x]$.
 The standard conditional expectation argument yields that the local-martingale $e^{ -Z_x} $ is a true $(\mathscr{G}_r)$-martingale under $\mathbf{P}$.
 The equality (\ref{AffineRepLap}) can be obtained immediately from the facts that
 \beqnn
 Z_x(x)= \lambda\cdot  X_\zeta(x) + g*X_\zeta(x)\geq 0
 \quad\mbox{and}\quad
 \mathbf{E}\big[e^{-Z_x(x)}\big]= \mathbf{E}\big[e^{-Y_x(0)}\big].
 \eeqnn 
 \qed
 
 
 \textit{\textbf{Proof of Theorem~???.}} Note that $e^{-Z_x(t)}= e^{-Y_x(0)}\cdot \mathcal{E}_{U_x}(t)$ for $t\in[0,x]$. 
 By Lemma~??, the process $e^{-Z_x}$ is a true $(\mathscr{F}_t)$-martingale. 
 Moreover, the equation ??? with $t=x$ shows that
 \beqnn
 Z_x(x)= \lambda X_\zeta(x)+ g* X_\zeta(x).
 \eeqnn
 Taking expectations on both sides of ???, we have 
 \beqnn
 \mathbf{E}\Big[ \exp\big\{-\lambda L^\xi_\zeta(x)- g* L^\xi_\zeta(x)\big\} \Big]
 = \mathbf{E}\big[ e^{-Z_x(x)} \big]
 = \mathbf{E}\big[ e^{-Y_x(0)} \big].
 \eeqnn
 By ??? and the exponential formula of stochastic integral with respect to Poisson random measure; see \cite[p.8]{Bertoin1996},  
 \beqnn
  \mathbf{E}\big[ e^{-Y_x(0)} \big]
 %= \mathbf{E}\bigg[\exp\Big\{ -\zeta \cdot c \cdot V^g_\lambda(x)  - \int_0^\zeta\int_0^\infty \Big( \int_{(x-y)^+}^x V^g_\lambda (r)dr \Big) \, N_0(dz, dy)  \Big\} \bigg]\cr
 \ar=\ar \exp\Big\{  -\zeta \cdot c\cdot V^g_\lambda(x)  \Big\}\cdot  \mathbf{E}\bigg[\exp\Big\{ - \int_0^\zeta\int_0^\infty \Big( \int_{(x-y)^+}^x V^g_\lambda (r)dr \Big) \, N_0(dz, dy)  \Big\} \bigg]\cr
 \ar=\ar \exp\bigg\{  -\zeta \cdot c\cdot V^g_\lambda(x) -\int_0^\infty \Big(1- \exp\Big\{-\int_{(x-s-y)^+}^{x-s} V^g_\lambda(r)dr\Big\} \Big) \bar\nu(y)dy  \bigg\}
 \eeqnn
 and hence the representation ??? holds.
 \qed 
  
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 
 

==> MainR.tex <==
 \section{Main results}
 \label{Sec.MainR}
 \setcounter{equation}{0}
 
 
 
 
 
  
 
 
 
   
 \begin{theorem}
 For any $T\geq 0$ and $\sigma$-finite measure $\mu(dx)$ on $\mathbb{R}_+$, the following hold.
 \begin{enumerate}
  \item[(1)] For any $\beta\in\mathbb{R}$, the nonlinear Volterra equation \eqref{NonlinearVolterra} is equivalent to 
  \beqlb\label{NonlinearVolterra02}
  V_\mu (t) =   W'_\beta*d\mu(t) + \big(\beta  V^g_\lambda-\boldsymbol{\mathcal{R}}\circ  V_\mu\big) *W'_\beta(t) ,\quad t\geq 0.
  \eeqlb
 	
  \item[(2)] The nonlinear Volterra equation \eqref{NonlinearVolterra} has a unique  global solution $V_\mu \in D(\mathbb{R}_+;\mathbb{R}_+) $ such that 
  \beqlb\label{eqn.211}
  0\leq V_\mu(t) \leq \frac{\mu([0,t])}{c},\quad t\geq 0.
  \eeqlb
   
  \item[(3)] The process  $Z_T:=\{Z_T(t):t\in[0,T] \}$ with
  \beqnn
  Z_T(t):= \mathbf{E}\big[  X_\zeta*d\mu(T) \,\big|\, \mathscr{F}_t \big] - \int_t^T \big(\boldsymbol{\mathcal{R}}\circ V_\mu\big) (T-s) \mathbf{E}\big[  X_\zeta(s) \,\big|\, \mathscr{F}_t \big] ds  
  \eeqnn
  is a continuous $(\mathscr{F}_t)$-semimartingale. 
  
  \item[(4)] The process $e^{-Z_T}:=\{ e^{-Z_T(t)}: t\in[0,T]  \} $ is a continuous $(\mathscr{F}_t)$-martingale. 
  
  \item[(5)] The Laplace functional of the process $L^\xi_\zeta$ admits the representation
  \beqnn
  \mathbf{E}\big[ \exp\big\{-  L^\xi_\zeta *d\mu(T) \big\} \big]
  = \mathbf{E}\big[ \exp\big\{ -Z_T(T) \big\} \big] 
  = \exp\big\{  -\zeta \cdot \boldsymbol{\mathcal{F}}\circ V_\mu(T)   \big\}, 
  \eeqnn
  where $\boldsymbol{\mathcal{F}}$ is a nonlinear operator acting on a locally integrable
  function $f$ by
  \beqnn
  \boldsymbol{\mathcal{F}}\circ f(t)
  \ar=\ar c\cdot f(t) + \int_0^\infty \Big(1- \exp\Big\{-\int_{(t-y)^+}^{t} f(r)dr\Big\}   \Big) \bar\nu(y)dy . 
  \eeqnn 
 \end{enumerate}
 	
 \end{theorem}
 
 \begin{theorem} 
 The following hold.
 \begin{enumerate}
 \item[(1)]  For any $\lambda \geq 0$ and $g\in L^\infty(\mathbb{R}_+;\mathbb{R}_+)$, the generalized Volterra-Riccati equation (??) has a unique global solution $V^\lambda_g \in C(\mathbb{R}_+;\mathbb{R}_+)\cap C^2\big((0,\infty);\mathbb{R}_+\big)$.
 	
 \item[(2)] For any $K_1,K_2>0$ and $T\geq 0$, there exists a constant $C>0$ such that for any $\lambda_1,\lambda_2\in[0,K_1]$ and $g_1,g_2 \in L^\infty(\mathbb{R}_+;\mathbb{R}_+) $ with $\big\|g_1\big\|_{L^\infty_T}, \big\|g_2\big\|_{L^\infty_T}\in[0,K_2]$,
 \beqnn
 \sup_{t\in[0,T]} \big| V^{g_1}_{\lambda_1} (t) -V^{g_2}_{\lambda_2} (t)\big|
 \leq C\cdot \Big(\big| \lambda_1-\lambda_2 \big| + \big\|g_1-g_2\big\|_{L^\infty_T}\Big).
 \eeqnn
 \end{enumerate}
 \end{theorem}
 
 
 
  

==> Regularity.tex <==
 \section{Regularity and maximal inequality}
 \label{Sec.Regularity}
 \setcounter{equation}{0}
 
 We now prove the uniform upper bounds for all moments of the sequence $\{ X^{(n)}_\zeta\}_{n\geq1}$  by using the following useful auxiliary result about the moment estimates for stochastic Volterra integrals with respect to a Poisson random measure given by 
 \beqlb
  B(f,t):= \int_0^t  \int_0^{X(s-)} f(t-s)B(ds,dz),\quad t\geq 0,
 \eeqlb
 for a measurable function $f$ on $\mathbb{R}_+$, a $(\mathscr{F}_t)$-predictable non-negative process $\{X(t):t\geq 0\} \in D(\mathbb{R}_+;\mathbb{R}_+)$ and a $(\mathscr{F}_t)$-Gaussian white noise $B(ds,dz)$ on $(0,\infty)^2$ with intensity $\gamma\cdot ds\, dz$ and $\nu_1(dy)$ being a $\sigma$-finite measure on $(0,\infty)$. 
 \begin{proposition} 
 	For two constants $p\geq 1$ and $T>0$, assume that
 	\beqnn
 	\sup_{t\in[0,T]}\mathbf{E}\Big[\big|X(t)\big|^{p}\Big]<\infty
 	\quad \mbox{and}\quad 
 	\int_0^T ds \int_0^\infty \big|f(s)\big|^{2p}ds <\infty.
 	\eeqnn
 	Then there exists a constant $C>0$ depending only on $p$ such that
 	\beqlb \label{BDG}
 	\sup_{t\in[0,T]}\mathbf{E}\Big[ \big| \widetilde{N}_1(f,t) \big|^{2p}  \Big] 
 	%\ar\leq\ar\mathbf{E}\Big[ \sup_{t\in[0,T]}\Big| \int_0^t \int_0^\infty \int_0^{X(s)} f(s,y)\widetilde{N}_1(ds,dy,dz) \Big|^{2p}  \Big]\cr
 	\ar\leq\ar C  \cdot \sup_{t\in[0,T]}\mathbf{E} \Big[\big|X(t)\big|^p \Big] \cdot \Bigg| \int_0^T  \int_0^\infty\big|f(s,y)\big|^{2} \nu_1(dy)  ds\Bigg|^{p} \cr
 	\ar\ar + C \cdot \sup_{t\in[0,T]}\mathbf{E}\Big[\big|X(t)\big|\Big]\cdot \int_0^T  \int_0^\infty\big|f(s,y)\big|^{2p} \nu_1(dy)  ds .
 	\eeqlb 
 \end{proposition}
 \proof For each $t_0\in[0,T]$, we consider an auxiliary martingale $\widetilde{N}_{t_0}(f,\cdot)$ defined by
 \beqnn
 \widetilde{N}_{t_0} (f,t) := \int_0^t \int_0^\infty \int_0^{X(s-)} f(t_0-s,y)\widetilde{N}_1(ds,dy,dz),\quad t\geq 0.
 \eeqnn
 It is obvious that $ \widetilde{N}_1 (f,t_0)\overset{\rm a.s.}=\widetilde{N}_{t_0}(f,t_0)$ and hence 
 \beqnn
 \sup_{t\in[0,T]}\mathbf{E}\Big[ \big| \widetilde{N}_1(f,t) \big|^{2p}  \Big]  =
 \sup_{t_0\in[0,T]}\mathbf{E}\Big[ \big|\widetilde{N}_{t_0} (f,t_0) \big|^{2p}  \Big] .
 \eeqnn
 By using Theorem~D.1 in \cite{Xu2024b} and then the change of variables to the last expectation, we have 
 \beqnn
 \mathbf{E}\Big[ \big|\widetilde{N}_{t_0} (f,t_0) \big|^{2p}  \Big] 
 \ar\leq\ar 
 \mathbf{E}\Big[ \sup_{t\in[0,t_0]} \big|\widetilde{N}_{t_0} (f,t) \big|^{2p}  \Big]\cr
 \ar\leq\ar 
 C  \cdot \sup_{t\in[0,t_0]}\mathbf{E} \Big[\big|X(t)\big|^p \Big] \cdot \Bigg| \int_0^{t_0}  \int_0^\infty\big|f(t_0-s,y)\big|^{2} \nu_1(dy)  ds\Bigg|^{p} \cr
 \ar\ar + C \cdot \sup_{t\in[0,t_0]}\mathbf{E}\Big[\big|X(t)\big|\Big]\cdot \int_0^{t_0}  \int_0^\infty\big|f(t_0-s,y)\big|^{2p} \nu_1(dy)  ds \cr
 \ar\leq\ar C  \cdot \sup_{t\in[0,T]}\mathbf{E} \Big[\big|X(t)\big|^p \Big] \cdot \Bigg| \int_0^T  \int_0^\infty\big|f(s,y)\big|^{2} \nu_1(dy)  ds\Bigg|^{p} \cr
 \ar\ar + C \cdot \sup_{t\in[0,T]}\mathbf{E}\Big[\big|X(t)\big|\Big]\cdot \int_0^T  \int_0^\infty\big|f(s,y)\big|^{2p} \nu_1(dy)  ds ,
 \eeqnn
 for some constant $C$ depending only on $p$. 
 Hence the desired inequality \eqref{BDG} holds. 
 \qed 
 
 
 \begin{corollary}
  For each $p\geq 0$, there exists a constant $C>0$  such that for any $t\geq 0$,
  \beqlb\label{eqn.41888}
  \mathbf{E}\Big[\big| X_\zeta(t) \big|^p  \Big] 
  \leq C\cdot (\zeta \vee \zeta^p) \cdot (1+t)^p. 
  \eeqlb  
 \end{corollary}
 \proof By using the monotone convergence theorem, the continuous mapping theorem and then Lemma~???, ???, 
 \beqnn
 \mathbf{E}\Big[\big| X_\zeta(t) \big|^p  \Big]
  = \lim_{K\to\infty} \mathbf{E}\Big[\big| X_\zeta(t) \big|^p \wedge K \Big]  
 \ar\leq\ar \lim_{K\to\infty} \lim_{n\to\infty}\mathbf{E}\Big[\big| X_\zeta^{(n)}(t)  \big|^p \wedge K \Big] 
 \leq  \sup_{n\geq 1}\mathbf{E}\Big[\big| X_\zeta^{(n)}(t)  \big|^p  \Big],
 \eeqnn
 which can be bounded by $C\cdot (\zeta \vee \zeta^p) \cdot (1+t)^p$ uniformly in $t\geq 0$. 
 \qed 
 
 \beqnn
 X_\zeta(t)\ar=\ar \zeta \Big(1-(b+\beta)W_\beta(t)\Big)    + 	\beta \cdot W'_\beta * X_\zeta(t) +\widetilde{\mathbf{I}}_{\nu,\beta}(t)   + \mathbf{J}_{c,\beta}(t) +\mathbf{J}_{\nu,\beta}(t),
 \eeqnn
 where 
 \beqnn
 \widetilde{\mathbf{I}}_{\nu,\beta}(t) \ar:=\ar  \int_0^\zeta\int_0^\infty \big( W_\beta(t)-W_\beta(t-y) \big) \, \widetilde{N}_0(dz, dy)  
 \eeqnn
 
 \begin{lemma}
 	For any $\beta \in \mathbb{R}$, we have uniformly in $\delta \geq 0$, 
 	\beqnn
 	\sup_{t\geq 0}\Big| \zeta \big(1-(b+\beta)W_\beta(t+\delta)\big) -\zeta \big(1-(b+\beta)W_\beta(t)\big)\Big|
  	\leq \zeta\cdot \frac{|b+\beta|}{c} \cdot \delta . 
 	\eeqnn 
 \end{lemma}
 \proof The desired upper bound follows directly from the monotonicity and differentiability of $W$ and \eqref{eqn.201}, i.e.,  uniformly in $t,\delta\geq 0$, 
 \beqnn
 \lefteqn{\Big| \zeta \big(1-(b+\beta)W_\beta(t+\delta)\big) -\zeta \big(1-(b+\beta)W_\beta(t)\big)\Big|}\ar\ar\cr
 \ar=\ar \zeta \cdot |b+\beta|\cdot \Big| W_\beta(t+\delta) -  W_\beta(t)\Big|
 =\zeta \cdot |b+\beta|\cdot \int_t^{t+\delta} W'(r)dr
 \leq \zeta\cdot \frac{|b+\beta|}{c} \cdot \delta.
 \eeqnn 
 \qed 
 
 \begin{lemma}
 For each $\beta \in \mathbb{R}$ such that $\beta+ b>0$, there exists a constant $C>0$ such that for any $\delta >0$ and $t\geq 0$,
 \beqnn
  \mathbf{E}\Big[ \big|\widetilde{\mathbf{I}}_{\nu,\beta}(t+\delta) - \widetilde{\mathbf{I}}_{\nu,\beta}(t)  \big|^{2p}  \Big] 
  \leq C\cdot (\zeta \vee \zeta^p) \cdot (1+\delta)^p \cdot \delta ^p.
 \eeqnn
 \end{lemma}
 \proof Applying \eqref{BDG} to ???, we have 
 \beqnn
 \mathbf{E}\Big[ \big|\widetilde{\mathbf{I}}_{\nu,\beta}(t+\delta) - \widetilde{\mathbf{I}}_{\nu,\beta}(t)  \big|^{2p}  \Big] 
 \ar\leq\ar C\cdot \zeta^p \cdot\Bigg( \int_0^\infty \Big|\int_{t+\delta-y}^{t+\delta} W'_\beta(r)dr  - \int_{t-y}^{t} W'_\beta(r)dr \Big|^2 \bar\nu(y)\,dy\Bigg)^p \cr
 \ar\ar + C\cdot \zeta \cdot  \int_0^\infty \Big|\int_{t+\delta-y}^{t+\delta} W'_\beta(r)dr  - \int_{t-y}^{t} W'_\beta(r)dr \Big|^{2p} \bar\nu(y)\,dy .
 \eeqnn
 Notice that 
 \beqnn
 \Big|\int_{t+\delta-y}^{t+\delta} W'_\beta(r)dr  - \int_{t-y}^{t} W'_\beta(r)dr \Big|
 \leq \frac{2}{c} \cdot ( \delta\wedge y) 
 \eeqnn
 and hence 
 \beqnn
 \mathbf{E}\Big[ \big|\widetilde{\mathbf{I}}_{\nu,\beta}(t+\delta) - \widetilde{\mathbf{I}}_{\nu,\beta}(t)  \big|^{2p}  \Big]
 \ar\leq\ar C\cdot \zeta^p \cdot\Bigg( \int_0^\infty   ( \delta\wedge y)^2 \bar\nu(y)\,dy\Bigg)^p 
  + C\cdot \zeta \cdot  \int_0^\infty  (\delta\wedge y)^{2p} \bar\nu(y)\,dy. 
 \eeqnn
 and uniformly in $\delta >0$, 
 \beqnn
 \int_0^\infty  (\delta\wedge y)^2 \bar\nu(y)\,dy
 \ar\leq\ar \delta \cdot \Big( \int_0^\delta y \bar\nu(y)\,dy  + \int_\delta^\infty  \delta  \bar\nu(y)\,dy  \Big)\cr
 \ar\leq\ar \delta \cdot \Big( \int_0^1 y \bar\nu(y)\,dy  + \delta \int_1^\infty \bar\nu(y)\,dy  \Big)
 \leq C\cdot (1+\delta) \cdot \delta.
 \eeqnn
 and
 \beqnn
 \int_0^\infty  (\delta\wedge y)^{2p} \bar\nu(y)\,dy
 \ar\leq\ar \delta^{2p-1} \cdot \Big( \int_0^\delta y \bar\nu(y)\,dy  + \int_\delta^\infty  \delta  \bar\nu(y)\,dy  \Big)\cr
 \ar\leq\ar  \delta^{2p-1} \cdot \Big( \int_0^1 y \bar\nu(y)\,dy  + \delta \int_1^\infty \bar\nu(y)\,dy  \Big)
 \leq C\cdot (1+\delta) \cdot  \delta^{2p-1}.
 \eeqnn
 Consequently, 
 \beqnn
 \ar\ar\mathbf{E}\Bigg[ \bigg| \int_0^\zeta \int_0^\infty \big( W_\beta(t+\delta)-W_\beta(t+\delta-y) \big) \, \widetilde{N}_0(dz, dy)- \int_0^\zeta\int_0^\infty \big( W_\beta(t)-W_\beta(t-y) \big) \, \widetilde{N}_0(dz, dy) \bigg|^{2p}  \Bigg] \cr
 \ar\leq\ar C \cdot \zeta^p \cdot  (1+\delta)^p \cdot \delta ^p  + C\cdot \zeta \cdot  (1+\delta) \cdot  \delta^{2p-1}
 \eeqnn
 \qed 
  
  
  
 \begin{lemma}
 For any $\beta\in\mathbb{R}$ such that $\beta+b>0$,  we have 
 \beqnn
  \mathbf{E}\Bigg[  \bigg|\int_0^{t+\delta}   W'_\beta(t+\delta-s) X_\zeta(s)ds - \int_0^t 	  W'_\beta(t-s) X_\zeta(s)ds \bigg|^{2p} \Bigg] \leq C\cdot \delta^p \cdot  (\zeta \vee \zeta^{2p})\cdot (1+t+\delta)^{3p}  
 \eeqnn
 	
 \end{lemma}
 \proof 
 \beqnn
 \ar\ar \Bigg|\int_0^{t+\delta}   W'_\beta(t+\delta-s) X_\zeta(s)ds - \int_0^t 	  W'_\beta(t-s) X_\zeta(s)ds \Bigg|^{2p} \cr
 \ar=\ar  \Bigg|\int_0^{t-\delta} \big(  W'_\beta(t+\delta-s)-  W'_\beta(t-s)\big) X_\zeta(s)ds \Bigg|^{2p}\cr
 \ar\leq\ar \Bigg|\int_0^{t+\delta} \big(  W'_\beta(t+\delta-s)-  W'_\beta(t-s)\big)^2\Bigg|^p\cdot \Bigg| \int_0^{t+\delta}\big|X_\zeta(s)\big|^2\,ds \Bigg|^{p}\cr
 \ar\leq\ar \Bigg|\int_0^{t+\delta} \big(  W'_\beta(s)-  W'_\beta(s-\delta)\big)^2ds\Bigg|^p\cdot  (t+\delta)^{p-1}\cdot \int_0^{t+\delta}\big|X_\zeta(s)\big|^{2p}\,ds   
 \eeqnn
 and hence 
 \beqnn
 \mathbf{E}\Bigg[  \bigg|\int_0^{t+\delta}   W'_\beta(t+\delta-s) X_\zeta(s)ds - \int_0^t 	  W'_\beta(t-s) X_\zeta(s)ds \bigg|^{2p} \Bigg]
 \leq C \cdot  (\zeta \vee \zeta^{2p})\cdot (1+t+\delta)^{3p} \cdot \delta^p. 
 \eeqnn
 \qed
 
 \begin{lemma}
 	For any $\beta\in\mathbb{R}$ such that $\beta+b>0$,  we have
 	\beqnn
 	\mathbf{E}\Big[\big|\mathbf{J}_{c,\beta}(t+\delta)- \mathbf{J}_{c,\beta}(t)\big|^{2p}\Big]
 	\leq C\cdot  (\zeta \vee \zeta^{p})\cdot (1+t+\delta)^{p}\cdot \delta^p . 
 	\eeqnn
 \end{lemma}
 \proof 
 \beqnn
 \mathbf{E}\Big[\big|\mathbf{J}_{c,\beta}(t+\delta)- \mathbf{J}_{c,\beta}(t)\big|^{2p}\Big]\ar\leq\ar C\cdot \mathbf{E}\Bigg[\bigg|2c\cdot\int_0^{t+\delta} X_\zeta(s)  \big( W'_\beta(t+\delta-s) - W'_\beta(t-s)\big)^2 \,  ds \bigg|^{p}\Bigg]\cr
 \ar\leq\ar C\cdot \Bigg|\int_0^{t+\delta}  \big( W'_\beta(t+\delta-s) - W'_\beta(t-s)\big)^2\,ds \Bigg|^{p-1}\cr
 \ar\ar \cdot \int_0^{t+\delta} \mathbf{E}\Big[ \big|X_\zeta(s)\big|^p \Big] \big( W'_\beta(t+\delta-s) - W'_\beta(t-s)\big)^2 \,  ds \cr
 \ar\leq\ar   C\cdot  (\zeta \vee \zeta^{p})\cdot (1+t+\delta)^{p}\cdot  \Bigg|\int_0^{t+\delta}  \big( W'_\beta(s) - W'_\beta(s-\delta)\big)^2\,ds \Bigg|^{p} \cr
 \ar\leq\ar  C\cdot  (\zeta \vee \zeta^{p})\cdot (1+t+\delta)^{p}\cdot \delta^p.
 \eeqnn
 \qed 
 
 \begin{lemma}
 	
 \beqnn
  \mathbf{E}\Big[\big|\mathbf{J}_{\nu,\beta}(t+\delta)- \mathbf{J}_{\nu,\beta}(t)\big|^{2p}\Big] \leq C\cdot (\zeta \vee \zeta^p)\cdot (1+t+\delta )^{3p} \cdot \delta^p.
 \eeqnn
 	
 \end{lemma}
 \proof 
 \beqnn
 \mathbf{J}_{\nu,\beta}(t+\delta)- \mathbf{J}_{\nu,\beta}(t)=\int_0^{t+\delta}\int_0^{X_\zeta(s)} \int_0^\infty \Big( \int_{t+\delta-s-y}^{t+\delta-s} W'_\beta(r)dr - \int_{t-s-y}^{t-s} W'_\beta(r)dr  \Big)\, \widetilde{N}_\nu(ds,dz,dy)
 \eeqnn
 By using \cite{BDG}, the change of variables and then Lemma~???, we have 
 \beqnn
 \mathbf{E}\Big[\big|\mathbf{J}_{\nu,\beta}(t+\delta)- \mathbf{J}_{\nu,\beta}(t)\big|^{2p}\Big]
 \ar\leq\ar C\cdot  \sup_{s\in[0,t+\delta]} \mathbf{E}\Big[ \big| X_\zeta(s)\big|^p \Big]\cdot \big|A_2(t,\delta)\big|^p\cr
 \ar\ar +  C\cdot  \sup_{s\in[0,t+\delta]} \mathbf{E}\Big[ \big| X_\zeta(s)\big|  \Big]\cdot A_{2p}(t,\delta)\cr
 \ar\leq\ar C\cdot (\zeta \vee \zeta^p)\cdot (1+t+\delta )^p  \cdot \big|A_2(t,\delta)\big|^p +  C\cdot   \zeta  \cdot (1+t+\delta ) \cdot A_{2p}(t,\delta)
 \eeqnn
 where 
 \beqnn
 A_{2k}(t,\delta)
 \ar:=\ar \int_{0}^{t+\delta} \int_0^\infty \Big( \int_{t+\delta-s-y}^{t+\delta-s} W'_\beta(r)dr - \int_{t-s-y}^{t-s} W'_\beta(r)dr  \Big)^{2k}\, ds\,\nu(dy)
 \eeqnn
 For $k=1$, by the change of variables and then H\"older's equality we have 
 \beqnn
 A_2(t,\delta)
 \ar=\ar \int_t^{t+\delta} \int_0^\infty \Big( \int_{t+\delta-s-y}^{t+\delta-s} W'_\beta(r)dr  \Big)^2\, ds\,\nu(dy)\cr
 \ar\ar + \int_{0}^t \int_0^\infty \Big( \int_{t+\delta-s-y}^{t+\delta-s} W'_\beta(r)dr - \int_{t-s-y}^{t-s} W'_\beta(r)dr  \Big)^2\, ds\,\nu(dy).
 \eeqnn
 The first term can be bounded by 
 \beqnn
 \int_t^{t+\delta} \int_0^\infty \Big( \int_{t+\delta-s-y}^{t+\delta-s} W'_\beta(r)dr  \Big)^2\, ds\,\nu(dy)
 \ar=\ar \int_0^{\delta} \int_0^\infty \Big( \int_{s-y}^{s} W'_\beta(r)dr  \Big)^2\, ds\,\nu(dy)\cr
 \ar\leq\ar \frac{1}{c^2}\int_0^{\delta} \int_0^\infty ( s\wedge y    )^2\, ds\,\nu(dy)\cr
 \ar\leq\ar \frac{\delta}{c^2}\cdot \int_0^\infty ( \delta\wedge y    )^2\, ds\,\nu(dy) 
 \leq C\cdot (1+\delta)^2 \cdot \delta.
 \eeqnn
 Moreover, by the change of variables 
 \beqnn
 \lefteqn{ \int_{0}^t \int_0^\infty \Big( \int_{t+\delta-s-y}^{t+\delta-s} W'_\beta(r)dr - \int_{t-s-y}^{t-s} W'_\beta(r)dr  \Big)^2\, ds\,\nu(dy)}\ar\ar\cr
 \ar=\ar  \int_{0}^t \int_0^\infty \Big( \int_{s+\delta-y}^{s+\delta} W'_\beta(r)dr - \int_{s-y}^{s} W'_\beta(r)dr  \Big)^2\, ds\,\nu(dy)\cr
 \ar=\ar \int_{0}^t \int_0^\infty \Big( \int_{s-y}^{s} \big( W'_\beta(r+\delta)- W'_\beta(r)\big) dr  \Big)^2\, ds\,\nu(dy)\cr
 \ar\leq\ar \int_{0}^t \int_0^\infty (s\wedge y) \int_{s-y}^{s} \big( W'_\beta(r+\delta)- W'_\beta(r)\big)^2 dr \, ds\,\nu(dy)\cr
 \ar=\ar \int_0^\infty \nu(dy) \int_{0}^t (s\wedge y) \int_{(s-y)^- }^0 \big( W'_\beta(r+\delta) \big)^2 dr \, ds\cr
 \ar\ar + \int_0^\infty \nu(dy) \int_{0}^t (s\wedge y) \int_{(s-y)^+}^t \big( W'_\beta(r+\delta)- W'_\beta(r)\big)^2 dr \, ds 
 \eeqnn
 Here 
 \beqnn
  \int_0^\infty \nu(dy) \int_{0}^t (s\wedge y) \int_{(s-y)^- }^0 \big( W'_\beta(r+\delta) \big)^2 dr \, ds
  \ar\leq\ar \frac{1}{c^2} \int_0^\infty \nu(dy) \int_{0}^t (s\wedge y) (\delta \wedge (y-s)^+)  \, ds \cr
  \ar=\ar \frac{1}{c^2}  \int_{0}^t (s\wedge y)\int_s^\infty  (\delta \wedge (y-s) ) \nu(dy) \, ds\cr
  \ar\leq\ar \frac{\delta}{c^2}  \int_{0}^t (s\wedge y)   \bar\nu(s) \, ds 
  \leq C\cdot (1+t)^2\cdot \delta. 
 \eeqnn
 and 
 \beqnn
 \lefteqn{\int_0^\infty \nu(dy) \int_{0}^t (s\wedge y) \int_{(s-y)^+}^t \big( W'_\beta(r+\delta)- W'_\beta(r)\big)^2 dr \, ds }\ar\ar\cr
 \ar=\ar \int_0^\infty \nu(dy) \int_{0}^t  \big( W'_\beta(s+\delta)- W'_\beta(s)\big)^2 \int_{s}^{(s+y)\wedge t} (r\wedge y) dr \, ds\cr
 \ar=\ar \int_0^\infty (t\wedge y)^2 \nu(dy) \cdot \int_{0}^t \big( W'_\beta(s+\delta)- W'_\beta(s)\big)^2   ds\cr
 \ar\leq\ar C\cdot (1+t+\delta)^2\cdot \delta. 
 \eeqnn
 In conclusion, we have 
 \beqnn
  A_2(t,\delta) 
  \leq C\cdot (1+t+\delta)^2\cdot \delta.
 \eeqnn
 Moreover,  Notice that 
 \beqnn
 \Big| \int_{s-y}^{s} W'_\beta(r)dr - \int_{s-\delta-y}^{s-\delta} W'_\beta(r)dr  \Big|
 \ar\leq\ar \frac{2}{c}\cdot (\delta\wedge y)
 \eeqnn
 we have 
 \beqnn
  A_{2k}(t,\delta)\leq \Big(\frac{2\delta}{c} \Big)^{2k-2} \cdot A_2(t,\delta)
  \leq C\cdot(1+t+\delta)^2\cdot \delta^{2k-1}
 \eeqnn
 and hence 
 \beqnn
 \mathbf{E}\Big[\big|\mathbf{J}_{\nu,\beta}(t+\delta)- \mathbf{J}_{\nu,\beta}(t)\big|^{2p}\Big]
 \ar\leq\ar  C\cdot (\zeta \vee \zeta^p)\cdot (1+t+\delta )^{3p}  \cdot   \delta^p \cr\ar\ar +  C\cdot   \zeta  \cdot  (1+t+\delta)^3\cdot \delta^{2p-1} \cr
 \ar\leq\ar C\cdot (\zeta \vee \zeta^p)\cdot (1+t+\delta )^{3p} \cdot \delta^p
 \eeqnn
 
 
 
 
 
 Armed with the preceding lemmas, we are now ready to prove Theorem~???. 
 The proof will need the Garsia-Rodemich-Rumsey inequality; see Lemma~1.1 in \cite{GarsiaRodemichRumseyRosenblatt1970} with $\psi(u)=|u|^p$ and $p(u)=|u|^{q+1/p}$ for $q>1/p$.
 It states that for a continuous function $f$ on $\mathbb{R}_+$, there exists a constant $C_{p,q}>0$ such that for any $x_2>x_1\geq 0$, 
 \beqlb\label{eqn.405}
 \big|f(x_2)-f(x_1) \big| \leq C_{p,q} \cdot \big| x_2-x_1\big|^{pq-1} \int_{x_1}^{x_2} ds \int_{x_1}^{x_2} \frac{|f(s)-f(r)|}{|s-r|^{pq+1}}dr.
 \eeqlb

==> SVECharacterization.tex <==
  \section{SVE for $L^\xi_\zeta$: Characterization}
 \label{Sec.SVECharacterization}
 \setcounter{equation}{0}
 
 
